Deformations of Gentle $A_\infty$-Algebras

In this paper we calculate the Hochschild cohomology of gentle $A_\infty$-algebras of arc collections on marked surfaces without boundary components. When the underlying arc collection has no loops or two-cycles, we show that the dgla structure of the Hochschild complex is formal and give an explicit realization of all deformations up to gauge equivalence.

==> filetree.tex <==
\input{new_intro.tex}
\input{orbigons.tex}
\input{new_hochschild.tex}

